Active Learning and Novel Model Calibration Measurements for Automated Visual Inspection in Manufacturing

Quality control is a crucial activity performed by manufacturing enterprises to ensure that their products meet quality standards and avoid potential damage to the brand's reputation. The decreased cost of sensors and connectivity enabled increasing digitalization of manufacturing. In addition, artificial intelligence enables higher degrees of automation, reducing overall costs and time required for defect inspection. This research compares three active learning approaches, having single and multiple oracles, to visual inspection. Six new metrics are proposed to assess the quality of calibration without the need for ground truth. Furthermore, this research explores whether existing calibrators can improve their performance by leveraging an approximate ground truth to enlarge the calibration set. The experiments were performed on real-world data provided by Philips Consumer Lifestyle BV. Our results show that the explored active learning settings can reduce the data labeling effort by between three and four percent without detriment to the overall quality goals, considering a threshold of p=0.95. Furthermore, the results show that the proposed calibration metrics successfully capture relevant information otherwise available to metrics used up to date only through ground truth data. Therefore, the proposed metrics can be used to estimate the quality of models' probability calibration without committing to a labeling effort to obtain ground truth data.

==> sn-sample-bib.tex <==
%% BioMed_Central_Bib_Style_v1.01

\begin{thebibliography}{69}
% BibTex style file: bmc-mathphys.bst (version 2.1), 2014-07-24
\ifx \bisbn   \undefined \def \bisbn  #1{ISBN #1}\fi
\ifx \binits  \undefined \def \binits#1{#1}\fi
\ifx \bauthor  \undefined \def \bauthor#1{#1}\fi
\ifx \batitle  \undefined \def \batitle#1{#1}\fi
\ifx \bjtitle  \undefined \def \bjtitle#1{#1}\fi
\ifx \bvolume  \undefined \def \bvolume#1{\textbf{#1}}\fi
\ifx \byear  \undefined \def \byear#1{#1}\fi
\ifx \bissue  \undefined \def \bissue#1{#1}\fi
\ifx \bfpage  \undefined \def \bfpage#1{#1}\fi
\ifx \blpage  \undefined \def \blpage #1{#1}\fi
\ifx \burl  \undefined \def \burl#1{\textsf{#1}}\fi
\ifx \doiurl  \undefined \def \doiurl#1{\url{https://doi.org/#1}}\fi
\ifx \betal  \undefined \def \betal{\textit{et al.}}\fi
\ifx \binstitute  \undefined \def \binstitute#1{#1}\fi
\ifx \binstitutionaled  \undefined \def \binstitutionaled#1{#1}\fi
\ifx \bctitle  \undefined \def \bctitle#1{#1}\fi
\ifx \beditor  \undefined \def \beditor#1{#1}\fi
\ifx \bpublisher  \undefined \def \bpublisher#1{#1}\fi
\ifx \bbtitle  \undefined \def \bbtitle#1{#1}\fi
\ifx \bedition  \undefined \def \bedition#1{#1}\fi
\ifx \bseriesno  \undefined \def \bseriesno#1{#1}\fi
\ifx \blocation  \undefined \def \blocation#1{#1}\fi
\ifx \bsertitle  \undefined \def \bsertitle#1{#1}\fi
\ifx \bsnm \undefined \def \bsnm#1{#1}\fi
\ifx \bsuffix \undefined \def \bsuffix#1{#1}\fi
\ifx \bparticle \undefined \def \bparticle#1{#1}\fi
\ifx \barticle \undefined \def \barticle#1{#1}\fi
\bibcommenthead
\ifx \bconfdate \undefined \def \bconfdate #1{#1}\fi
\ifx \botherref \undefined \def \botherref #1{#1}\fi
\ifx \url \undefined \def \url#1{\textsf{#1}}\fi
\ifx \bchapter \undefined \def \bchapter#1{#1}\fi
\ifx \bbook \undefined \def \bbook#1{#1}\fi
\ifx \bcomment \undefined \def \bcomment#1{#1}\fi
\ifx \oauthor \undefined \def \oauthor#1{#1}\fi
\ifx \citeauthoryear \undefined \def \citeauthoryear#1{#1}\fi
\ifx \endbibitem  \undefined \def \endbibitem {}\fi
\ifx \bconflocation  \undefined \def \bconflocation#1{#1}\fi
\ifx \arxivurl  \undefined \def \arxivurl#1{\textsf{#1}}\fi
\csname PreBibitemsHook\endcsname

%%% 1
\bibitem{yang2020using}
\begin{barticle}
\bauthor{\bsnm{Yang}, \binits{J.}},
\bauthor{\bsnm{Li}, \binits{S.}},
\bauthor{\bsnm{Wang}, \binits{Z.}},
\bauthor{\bsnm{Dong}, \binits{H.}},
\bauthor{\bsnm{Wang}, \binits{J.}},
\bauthor{\bsnm{Tang}, \binits{S.}}:
\batitle{Using deep learning to detect defects in manufacturing: a
  comprehensive survey and current challenges}.
\bjtitle{Materials}
\bvolume{13}(\bissue{24}),
\bfpage{5755}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 2
\bibitem{kurniati2015quality}
\begin{barticle}
\bauthor{\bsnm{Kurniati}, \binits{N.}},
\bauthor{\bsnm{Yeh}, \binits{R.-H.}},
\bauthor{\bsnm{Lin}, \binits{J.-J.}}:
\batitle{Quality inspection and maintenance: the framework of interaction}.
\bjtitle{Procedia manufacturing}
\bvolume{4},
\bfpage{244}--\blpage{251}
(\byear{2015})
\end{barticle}
\endbibitem

%%% 3
\bibitem{wuest2014approach}
\begin{barticle}
\bauthor{\bsnm{Wuest}, \binits{T.}},
\bauthor{\bsnm{Irgens}, \binits{C.}},
\bauthor{\bsnm{Thoben}, \binits{K.-D.}}:
\batitle{An approach to monitoring quality in manufacturing using supervised
  machine learning on product state data}.
\bjtitle{Journal of Intelligent Manufacturing}
\bvolume{25}(\bissue{5}),
\bfpage{1167}--\blpage{1180}
(\byear{2014})
\end{barticle}
\endbibitem

%%% 4
\bibitem{newman1995survey}
\begin{barticle}
\bauthor{\bsnm{Newman}, \binits{T.S.}},
\bauthor{\bsnm{Jain}, \binits{A.K.}}:
\batitle{A survey of automated visual inspection}.
\bjtitle{Computer vision and image understanding}
\bvolume{61}(\bissue{2}),
\bfpage{231}--\blpage{262}
(\byear{1995})
\end{barticle}
\endbibitem

%%% 5
\bibitem{zheng2020defect}
\begin{barticle}
\bauthor{\bsnm{Zheng}, \binits{Z.}},
\bauthor{\bsnm{Zhang}, \binits{S.}},
\bauthor{\bsnm{Yu}, \binits{B.}},
\bauthor{\bsnm{Li}, \binits{Q.}},
\bauthor{\bsnm{Zhang}, \binits{Y.}}:
\batitle{Defect inspection in tire radiographic image using concise semantic
  segmentation}.
\bjtitle{IEEE Access}
\bvolume{8},
\bfpage{112674}--\blpage{112687}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 6
\bibitem{vergara2014automatic}
\begin{bchapter}
\bauthor{\bsnm{Vergara-Villegas}, \binits{O.O.}},
\bauthor{\bsnm{Cruz-S{\'a}nchez}, \binits{V.G.}},
\bauthor{\bsnm{Jes{\'u}s~Ochoa-Dom{\'\i}nguez}, \binits{H.d.}},
\bauthor{\bsnm{Jes{\'u}s~Nandayapa-Alfaro}, \binits{M.d.}},
\bauthor{\bsnm{Flores-Abad}, \binits{{\'A}.}}:
\bctitle{Automatic product quality inspection using computer vision systems}.
In: \bbtitle{Lean Manufacturing in the Developing World},
pp. \bfpage{135}--\blpage{156}.
\bpublisher{Springer}, \blocation{???}
(\byear{2014})
\end{bchapter}
\endbibitem

%%% 7
\bibitem{selvi2017effective}
\begin{barticle}
\bauthor{\bsnm{Selvi}, \binits{S.S.T.}},
\bauthor{\bsnm{Nasira}, \binits{G.}}:
\batitle{An effective automatic fabric defect detection system using digital
  image processing}.
\bjtitle{J. Environ. Nanotechnol}
\bvolume{6}(\bissue{1}),
\bfpage{79}--\blpage{85}
(\byear{2017})
\end{barticle}
\endbibitem

%%% 8
\bibitem{see2012visual}
\begin{botherref}
\oauthor{\bsnm{See}, \binits{J.E.}}:
Visual inspection: a review of the literature.
Sandia Report SAND2012-8590, Sandia National Laboratories, Albuquerque, New
  Mexico
(2012)
\end{botherref}
\endbibitem

%%% 9
\bibitem{cullinane2013job}
\begin{barticle}
\bauthor{\bsnm{Cullinane}, \binits{S.-J.}},
\bauthor{\bsnm{Bosak}, \binits{J.}},
\bauthor{\bsnm{Flood}, \binits{P.C.}},
\bauthor{\bsnm{Demerouti}, \binits{E.}}:
\batitle{Job design under lean manufacturing and its impact on employee
  outcomes}.
\bjtitle{Organizational Psychology Review}
\bvolume{3}(\bissue{1}),
\bfpage{41}--\blpage{61}
(\byear{2013})
\end{barticle}
\endbibitem

%%% 10
\bibitem{kujawinska2016role}
\begin{bchapter}
\bauthor{\bsnm{Kujawi{\'n}ska}, \binits{A.}},
\bauthor{\bsnm{Vogt}, \binits{K.}},
\bauthor{\bsnm{Hamrol}, \binits{A.}}:
\bctitle{The role of human motivation in quality inspection of production
  processes}.
In: \bbtitle{Advances in Ergonomics of Manufacturing: Managing the Enterprise
  of the Future},
pp. \bfpage{569}--\blpage{579}.
\bpublisher{Springer}, \blocation{???}
(\byear{2016})
\end{bchapter}
\endbibitem

%%% 11
\bibitem{rai2021machine}
\begin{botherref}
\oauthor{\bsnm{Rai}, \binits{R.}},
\oauthor{\bsnm{Tiwari}, \binits{M.K.}},
\oauthor{\bsnm{Ivanov}, \binits{D.}},
\oauthor{\bsnm{Dolgui}, \binits{A.}}:
Machine learning in manufacturing and industry 4.0 applications.
Taylor \& Francis
(2021)
\end{botherref}
\endbibitem

%%% 12
\bibitem{zheng2021applications}
\begin{barticle}
\bauthor{\bsnm{Zheng}, \binits{T.}},
\bauthor{\bsnm{Ardolino}, \binits{M.}},
\bauthor{\bsnm{Bacchetti}, \binits{A.}},
\bauthor{\bsnm{Perona}, \binits{M.}}:
\batitle{The applications of industry 4.0 technologies in manufacturing
  context: a systematic literature review}.
\bjtitle{International Journal of Production Research}
\bvolume{59}(\bissue{6}),
\bfpage{1922}--\blpage{1954}
(\byear{2021})
\end{barticle}
\endbibitem

%%% 13
\bibitem{rovzanec2022human}
\begin{botherref}
\oauthor{\bsnm{Ro{\v{z}}anec}, \binits{J.M.}},
\oauthor{\bsnm{Novalija}, \binits{I.}},
\oauthor{\bsnm{Zajec}, \binits{P.}},
\oauthor{\bsnm{Kenda}, \binits{K.}},
\oauthor{\bsnm{Tavakoli}, \binits{H.}},
\oauthor{\bsnm{Suh}, \binits{S.}},
\oauthor{\bsnm{Veliou}, \binits{E.}},
\oauthor{\bsnm{Papamartzivanos}, \binits{D.}},
\oauthor{\bsnm{Giannetsos}, \binits{T.}},
\oauthor{\bsnm{Menesidou}, \binits{S.A.}}, et al.:
Human-centric artificial intelligence architecture for industry 5.0
  applications.
arXiv preprint arXiv:2203.10794
(2022)
\end{botherref}
\endbibitem

%%% 14
\bibitem{carvajal2019online}
\begin{barticle}
\bauthor{\bsnm{Carvajal~Soto}, \binits{J.}},
\bauthor{\bsnm{Tavakolizadeh}, \binits{F.}},
\bauthor{\bsnm{Gyulai}, \binits{D.}}:
\batitle{An online machine learning framework for early detection of product
  failures in an industry 4.0 context}.
\bjtitle{International Journal of Computer Integrated Manufacturing}
\bvolume{32}(\bissue{4-5}),
\bfpage{452}--\blpage{465}
(\byear{2019})
\end{barticle}
\endbibitem

%%% 15
\bibitem{chouchene2020artificial}
\begin{bchapter}
\bauthor{\bsnm{Chouchene}, \binits{A.}},
\bauthor{\bsnm{Carvalho}, \binits{A.}},
\bauthor{\bsnm{Lima}, \binits{T.M.}},
\bauthor{\bsnm{Charrua-Santos}, \binits{F.}},
\bauthor{\bsnm{Os{\'o}rio}, \binits{G.J.}},
\bauthor{\bsnm{Barhoumi}, \binits{W.}}:
\bctitle{Artificial intelligence for product quality inspection toward smart
  industries: quality control of vehicle non-conformities}.
In: \bbtitle{2020 9th International Conference on Industrial Technology and
  Management (ICITM)},
pp. \bfpage{127}--\blpage{131}
(\byear{2020}).
\bcomment{IEEE}
\end{bchapter}
\endbibitem

%%% 16
\bibitem{duan2012machine}
\begin{barticle}
\bauthor{\bsnm{Duan}, \binits{G.}},
\bauthor{\bsnm{Wang}, \binits{H.}},
\bauthor{\bsnm{Liu}, \binits{Z.}},
\bauthor{\bsnm{Chen}, \binits{Y.-W.}}:
\batitle{A machine learning-based framework for automatic visual inspection of
  microdrill bits in pcb production}.
\bjtitle{IEEE Transactions on Systems, Man, and Cybernetics, Part C
  (Applications and Reviews)}
\bvolume{42}(\bissue{6}),
\bfpage{1679}--\blpage{1689}
(\byear{2012})
\end{barticle}
\endbibitem

%%% 17
\bibitem{jiang2018fundamentals}
\begin{bchapter}
\bauthor{\bsnm{Jiang}, \binits{J.}},
\bauthor{\bsnm{Wong}, \binits{W.}}:
\bctitle{Fundamentals of common computer vision techniques for textile quality
  control}.
In: \bbtitle{Applications of Computer Vision in Fashion and Textiles},
pp. \bfpage{3}--\blpage{15}.
\bpublisher{Elsevier}, \blocation{???}
(\byear{2018})
\end{bchapter}
\endbibitem

%%% 18
\bibitem{villalba2019deep}
\begin{barticle}
\bauthor{\bsnm{Villalba-Diez}, \binits{J.}},
\bauthor{\bsnm{Schmidt}, \binits{D.}},
\bauthor{\bsnm{Gevers}, \binits{R.}},
\bauthor{\bsnm{Ordieres-Mer{\'e}}, \binits{J.}},
\bauthor{\bsnm{Buchwitz}, \binits{M.}},
\bauthor{\bsnm{Wellbrock}, \binits{W.}}:
\batitle{Deep learning for industrial computer vision quality control in the
  printing industry 4.0}.
\bjtitle{Sensors}
\bvolume{19}(\bissue{18}),
\bfpage{3987}
(\byear{2019})
\end{barticle}
\endbibitem

%%% 19
\bibitem{beltran2020external}
\begin{bchapter}
\bauthor{\bsnm{Beltr{\'a}n-Gonz{\'a}lez}, \binits{C.}},
\bauthor{\bsnm{Bustreo}, \binits{M.}},
\bauthor{\bsnm{Del~Bue}, \binits{A.}}:
\bctitle{External and internal quality inspection of aerospace components}.
In: \bbtitle{2020 IEEE 7th International Workshop on Metrology for AeroSpace
  (MetroAeroSpace)},
pp. \bfpage{351}--\blpage{355}
(\byear{2020}).
\bcomment{IEEE}
\end{bchapter}
\endbibitem

%%% 20
\bibitem{aggour2019artificial}
\begin{barticle}
\bauthor{\bsnm{Aggour}, \binits{K.S.}},
\bauthor{\bsnm{Gupta}, \binits{V.K.}},
\bauthor{\bsnm{Ruscitto}, \binits{D.}},
\bauthor{\bsnm{Ajdelsztajn}, \binits{L.}},
\bauthor{\bsnm{Bian}, \binits{X.}},
\bauthor{\bsnm{Brosnan}, \binits{K.H.}},
\bauthor{\bsnm{Kumar}, \binits{N.C.}},
\bauthor{\bsnm{Dheeradhada}, \binits{V.}},
\bauthor{\bsnm{Hanlon}, \binits{T.}},
\bauthor{\bsnm{Iyer}, \binits{N.}}, \betal:
\batitle{Artificial intelligence/machine learning in manufacturing and
  inspection: A ge perspective}.
\bjtitle{MRS Bulletin}
\bvolume{44}(\bissue{7}),
\bfpage{545}--\blpage{558}
(\byear{2019})
\end{barticle}
\endbibitem

%%% 21
\bibitem{silva2021classifier}
\begin{botherref}
\oauthor{\bsnm{Silva~Filho}, \binits{T.}},
\oauthor{\bsnm{Song}, \binits{H.}},
\oauthor{\bsnm{Perello-Nieto}, \binits{M.}},
\oauthor{\bsnm{Santos-Rodriguez}, \binits{R.}},
\oauthor{\bsnm{Kull}, \binits{M.}},
\oauthor{\bsnm{Flach}, \binits{P.}}:
Classifier calibration: How to assess and improve predicted class
  probabilities: a survey.
arXiv e-prints,
2112
(2021)
\end{botherref}
\endbibitem

%%% 22
\bibitem{rovzanec2022streaming}
\begin{barticle}
\bauthor{\bsnm{Ro{\v{z}}anec}, \binits{J.M.}},
\bauthor{\bsnm{Trajkova}, \binits{E.}},
\bauthor{\bsnm{Dam}, \binits{P.}},
\bauthor{\bsnm{Fortuna}, \binits{B.}},
\bauthor{\bsnm{Mladeni{\'c}}, \binits{D.}}:
\batitle{Streaming machine learning and online active learning for automated
  visual inspection.}
\bjtitle{IFAC-PapersOnLine}
\bvolume{55}(\bissue{2}),
\bfpage{277}--\blpage{282}
(\byear{2022})
\end{barticle}
\endbibitem

%%% 23
\bibitem{BRADLEY19971145}
\begin{barticle}
\bauthor{\bsnm{Bradley}, \binits{A.P.}}:
\batitle{The use of the area under the roc curve in the evaluation of machine
  learning algorithms}.
\bjtitle{Pattern Recognition}
\bvolume{30}(\bissue{7}),
\bfpage{1145}--\blpage{1159}
(\byear{1997}).
\doiurl{10.1016/S0031-3203(96)00142-2}
\end{barticle}
\endbibitem

%%% 24
\bibitem{schmitt2020predictive}
\begin{barticle}
\bauthor{\bsnm{Schmitt}, \binits{J.}},
\bauthor{\bsnm{B{\"o}nig}, \binits{J.}},
\bauthor{\bsnm{Borggr{\"a}fe}, \binits{T.}},
\bauthor{\bsnm{Beitinger}, \binits{G.}},
\bauthor{\bsnm{Deuse}, \binits{J.}}:
\batitle{Predictive model-based quality inspection using machine learning and
  edge cloud computing}.
\bjtitle{Advanced engineering informatics}
\bvolume{45},
\bfpage{101101}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 25
\bibitem{weiss2016continuous}
\begin{barticle}
\bauthor{\bsnm{Weiss}, \binits{S.M.}},
\bauthor{\bsnm{Dhurandhar}, \binits{A.}},
\bauthor{\bsnm{Baseman}, \binits{R.J.}},
\bauthor{\bsnm{White}, \binits{B.F.}},
\bauthor{\bsnm{Logan}, \binits{R.}},
\bauthor{\bsnm{Winslow}, \binits{J.K.}},
\bauthor{\bsnm{Poindexter}, \binits{D.}}:
\batitle{Continuous prediction of manufacturing performance throughout the
  production lifecycle}.
\bjtitle{Journal of Intelligent Manufacturing}
\bvolume{27}(\bissue{4}),
\bfpage{751}--\blpage{763}
(\byear{2016})
\end{barticle}
\endbibitem

%%% 26
\bibitem{park2016machine}
\begin{barticle}
\bauthor{\bsnm{Park}, \binits{J.-K.}},
\bauthor{\bsnm{Kwon}, \binits{B.-K.}},
\bauthor{\bsnm{Park}, \binits{J.-H.}},
\bauthor{\bsnm{Kang}, \binits{D.-J.}}:
\batitle{Machine learning-based imaging system for surface defect inspection}.
\bjtitle{International Journal of Precision Engineering and Manufacturing-Green
  Technology}
\bvolume{3}(\bissue{3}),
\bfpage{303}--\blpage{310}
(\byear{2016})
\end{barticle}
\endbibitem

%%% 27
\bibitem{ren2017generic}
\begin{barticle}
\bauthor{\bsnm{Ren}, \binits{R.}},
\bauthor{\bsnm{Hung}, \binits{T.}},
\bauthor{\bsnm{Tan}, \binits{K.C.}}:
\batitle{A generic deep-learning-based approach for automated surface
  inspection}.
\bjtitle{IEEE transactions on cybernetics}
\bvolume{48}(\bissue{3}),
\bfpage{929}--\blpage{940}
(\byear{2017})
\end{barticle}
\endbibitem

%%% 28
\bibitem{jian2017automatic}
\begin{barticle}
\bauthor{\bsnm{Jian}, \binits{C.}},
\bauthor{\bsnm{Gao}, \binits{J.}},
\bauthor{\bsnm{Ao}, \binits{Y.}}:
\batitle{Automatic surface defect detection for mobile phone screen glass based
  on machine vision}.
\bjtitle{Applied Soft Computing}
\bvolume{52},
\bfpage{348}--\blpage{358}
(\byear{2017})
\end{barticle}
\endbibitem

%%% 29
\bibitem{tsai2008defect}
\begin{barticle}
\bauthor{\bsnm{Tsai}, \binits{D.-M.}},
\bauthor{\bsnm{Lai}, \binits{S.-C.}}:
\batitle{Defect detection in periodically patterned surfaces using independent
  component analysis}.
\bjtitle{Pattern Recognition}
\bvolume{41}(\bissue{9}),
\bfpage{2812}--\blpage{2832}
(\byear{2008})
\end{barticle}
\endbibitem

%%% 30
\bibitem{kang2005surface}
\begin{bchapter}
\bauthor{\bsnm{Kang}, \binits{G.-W.}},
\bauthor{\bsnm{Liu}, \binits{H.-B.}}:
\bctitle{Surface defects inspection of cold rolled strips based on neural
  network}.
In: \bbtitle{2005 International Conference on Machine Learning and
  Cybernetics},
vol. \bseriesno{8},
pp. \bfpage{5034}--\blpage{5037}
(\byear{2005}).
\bcomment{IEEE}
\end{bchapter}
\endbibitem

%%% 31
\bibitem{yun2014defect}
\begin{barticle}
\bauthor{\bsnm{Yun}, \binits{J.P.}},
\bauthor{\bsnm{Choi}, \binits{D.-c.}},
\bauthor{\bsnm{Jeon}, \binits{Y.-j.}},
\bauthor{\bsnm{Park}, \binits{C.}},
\bauthor{\bsnm{Kim}, \binits{S.W.}}:
\batitle{Defect inspection system for steel wire rods produced by hot rolling
  process}.
\bjtitle{The International Journal of Advanced Manufacturing Technology}
\bvolume{70}(\bissue{9}),
\bfpage{1625}--\blpage{1634}
(\byear{2014})
\end{barticle}
\endbibitem

%%% 32
\bibitem{valavanis2010multiclass}
\begin{barticle}
\bauthor{\bsnm{Valavanis}, \binits{I.}},
\bauthor{\bsnm{Kosmopoulos}, \binits{D.}}:
\batitle{Multiclass defect detection and classification in weld radiographic
  images using geometric and texture features}.
\bjtitle{Expert Systems with Applications}
\bvolume{37}(\bissue{12}),
\bfpage{7606}--\blpage{7614}
(\byear{2010})
\end{barticle}
\endbibitem

%%% 33
\bibitem{cohen2020sub}
\begin{botherref}
\oauthor{\bsnm{Cohen}, \binits{N.}},
\oauthor{\bsnm{Hoshen}, \binits{Y.}}:
Sub-image anomaly detection with deep pyramid correspondences.
arXiv preprint arXiv:2005.02357
(2020)
\end{botherref}
\endbibitem

%%% 34
\bibitem{li2021cutpaste}
\begin{bchapter}
\bauthor{\bsnm{Li}, \binits{C.-L.}},
\bauthor{\bsnm{Sohn}, \binits{K.}},
\bauthor{\bsnm{Yoon}, \binits{J.}},
\bauthor{\bsnm{Pfister}, \binits{T.}}:
\bctitle{Cutpaste: Self-supervised learning for anomaly detection and
  localization}.
In: \bbtitle{Proceedings of the IEEE/CVF Conference on Computer Vision and
  Pattern Recognition},
pp. \bfpage{9664}--\blpage{9674}
(\byear{2021})
\end{bchapter}
\endbibitem

%%% 35
\bibitem{jezek2021deep}
\begin{bchapter}
\bauthor{\bsnm{Jezek}, \binits{S.}},
\bauthor{\bsnm{Jonak}, \binits{M.}},
\bauthor{\bsnm{Burget}, \binits{R.}},
\bauthor{\bsnm{Dvorak}, \binits{P.}},
\bauthor{\bsnm{Skotak}, \binits{M.}}:
\bctitle{Deep learning-based defect detection of metal parts: evaluating
  current methods in complex conditions}.
In: \bbtitle{2021 13th International Congress on Ultra Modern
  Telecommunications and Control Systems and Workshops (ICUMT)},
pp. \bfpage{66}--\blpage{71}
(\byear{2021}).
\bcomment{IEEE}
\end{bchapter}
\endbibitem

%%% 36
\bibitem{aiger2012phase}
\begin{bchapter}
\bauthor{\bsnm{Aiger}, \binits{D.}},
\bauthor{\bsnm{Talbot}, \binits{H.}}:
\bctitle{The phase only transform for unsupervised surface defect detection}.
In: \bbtitle{Emerging Topics In Computer Vision And Its Applications},
pp. \bfpage{215}--\blpage{232}.
\bpublisher{World Scientific}, \blocation{???}
(\byear{2012})
\end{bchapter}
\endbibitem

%%% 37
\bibitem{mujeeb2018unsupervised}
\begin{bchapter}
\bauthor{\bsnm{Mujeeb}, \binits{A.}},
\bauthor{\bsnm{Dai}, \binits{W.}},
\bauthor{\bsnm{Erdt}, \binits{M.}},
\bauthor{\bsnm{Sourin}, \binits{A.}}:
\bctitle{Unsupervised surface defect detection using deep autoencoders and data
  augmentation}.
In: \bbtitle{2018 International Conference on Cyberworlds (CW)},
pp. \bfpage{391}--\blpage{398}
(\byear{2018}).
\bcomment{IEEE}
\end{bchapter}
\endbibitem

%%% 38
\bibitem{zavrtanik2021draem}
\begin{bchapter}
\bauthor{\bsnm{Zavrtanik}, \binits{V.}},
\bauthor{\bsnm{Kristan}, \binits{M.}},
\bauthor{\bsnm{Sko{\v{c}}aj}, \binits{D.}}:
\bctitle{Draem-a discriminatively trained reconstruction embedding for surface
  anomaly detection}.
In: \bbtitle{Proceedings of the IEEE/CVF International Conference on Computer
  Vision},
pp. \bfpage{8330}--\blpage{8339}
(\byear{2021})
\end{bchapter}
\endbibitem

%%% 39
\bibitem{lewis1994heterogeneous}
\begin{bchapter}
\bauthor{\bsnm{Lewis}, \binits{D.D.}},
\bauthor{\bsnm{Catlett}, \binits{J.}}:
\bctitle{Heterogeneous uncertainty sampling for supervised learning}.
In: \bbtitle{Machine Learning Proceedings 1994},
pp. \bfpage{148}--\blpage{156}.
\bpublisher{Elsevier}, \blocation{???}
(\byear{1994})
\end{bchapter}
\endbibitem

%%% 40
\bibitem{cohn1994improving}
\begin{barticle}
\bauthor{\bsnm{Cohn}, \binits{D.}},
\bauthor{\bsnm{Atlas}, \binits{L.}},
\bauthor{\bsnm{Ladner}, \binits{R.}}:
\batitle{Improving generalization with active learning}.
\bjtitle{Machine learning}
\bvolume{15}(\bissue{2}),
\bfpage{201}--\blpage{221}
(\byear{1994})
\end{barticle}
\endbibitem

%%% 41
\bibitem{settles2009active}
\begin{botherref}
\oauthor{\bsnm{Settles}, \binits{B.}}:
Active learning literature survey
(2009)
\end{botherref}
\endbibitem

%%% 42
\bibitem{ren2020survey}
\begin{botherref}
\oauthor{\bsnm{Ren}, \binits{P.}},
\oauthor{\bsnm{Xiao}, \binits{Y.}},
\oauthor{\bsnm{Chang}, \binits{X.}},
\oauthor{\bsnm{Huang}, \binits{P.-Y.}},
\oauthor{\bsnm{Li}, \binits{Z.}},
\oauthor{\bsnm{Chen}, \binits{X.}},
\oauthor{\bsnm{Wang}, \binits{X.}}:
A survey of deep active learning.
arXiv preprint arXiv:2009.00236
(2020)
\end{botherref}
\endbibitem

%%% 43
\bibitem{beluch2018power}
\begin{bchapter}
\bauthor{\bsnm{Beluch}, \binits{W.H.}},
\bauthor{\bsnm{Genewein}, \binits{T.}},
\bauthor{\bsnm{N{\"u}rnberger}, \binits{A.}},
\bauthor{\bsnm{K{\"o}hler}, \binits{J.M.}}:
\bctitle{The power of ensembles for active learning in image classification}.
In: \bbtitle{Proceedings of the IEEE Conference on Computer Vision and Pattern
  Recognition},
pp. \bfpage{9368}--\blpage{9377}
(\byear{2018})
\end{bchapter}
\endbibitem

%%% 44
\bibitem{cordier2021active}
\begin{botherref}
\oauthor{\bsnm{Cordier}, \binits{A.}},
\oauthor{\bsnm{Das}, \binits{D.}},
\oauthor{\bsnm{Gutierrez}, \binits{P.}}:
Active learning using weakly supervised signals for quality inspection.
arXiv preprint arXiv:2104.02973
(2021)
\end{botherref}
\endbibitem

%%% 45
\bibitem{meng2020machine}
\begin{barticle}
\bauthor{\bsnm{Meng}, \binits{L.}},
\bauthor{\bsnm{McWilliams}, \binits{B.}},
\bauthor{\bsnm{Jarosinski}, \binits{W.}},
\bauthor{\bsnm{Park}, \binits{H.-Y.}},
\bauthor{\bsnm{Jung}, \binits{Y.-G.}},
\bauthor{\bsnm{Lee}, \binits{J.}},
\bauthor{\bsnm{Zhang}, \binits{J.}}:
\batitle{Machine learning in additive manufacturing: A review}.
\bjtitle{Jom}
\bvolume{72}(\bissue{6}),
\bfpage{2363}--\blpage{2377}
(\byear{2020})
\end{barticle}
\endbibitem

%%% 46
\bibitem{dai2018towards}
\begin{bchapter}
\bauthor{\bsnm{Dai}, \binits{W.}},
\bauthor{\bsnm{Mujeeb}, \binits{A.}},
\bauthor{\bsnm{Erdt}, \binits{M.}},
\bauthor{\bsnm{Sourin}, \binits{A.}}:
\bctitle{Towards automatic optical inspection of soldering defects}.
In: \bbtitle{2018 International Conference on Cyberworlds (CW)},
pp. \bfpage{375}--\blpage{382}
(\byear{2018}).
\bcomment{IEEE}
\end{bchapter}
\endbibitem

%%% 47
\bibitem{zajec2021towards}
\begin{bchapter}
\bauthor{\bsnm{Zajec}, \binits{P.}},
\bauthor{\bsnm{Ro{\v{z}}anec}, \binits{J.M.}},
\bauthor{\bsnm{Novalija}, \binits{I.}},
\bauthor{\bsnm{Fortuna}, \binits{B.}},
\bauthor{\bsnm{Mladeni{\'c}}, \binits{D.}},
\bauthor{\bsnm{Kenda}, \binits{K.}}:
\bctitle{Towards active learning based smart assistant for manufacturing}.
In: \bbtitle{IFIP International Conference on Advances in Production Management
  Systems},
pp. \bfpage{295}--\blpage{302}
(\byear{2021}).
\bcomment{Springer}
\end{bchapter}
\endbibitem

%%% 48
\bibitem{van2018active}
\begin{botherref}
\oauthor{\bparticle{van} \bsnm{Garderen}, \binits{K.}}:
Active learning for overlay prediction in semi-conductor manufacturing
(2018)
\end{botherref}
\endbibitem

%%% 49
\bibitem{cheeseman1985defense}
\begin{bchapter}
\bauthor{\bsnm{Cheeseman}, \binits{P.C.}}:
\bctitle{In defense of probability.}
In: \bbtitle{IJCAI},
vol. \bseriesno{85},
pp. \bfpage{1002}--\blpage{1009}
(\byear{1985})
\end{bchapter}
\endbibitem

%%% 50
\bibitem{cohen2004properties}
\begin{bchapter}
\bauthor{\bsnm{Cohen}, \binits{I.}},
\bauthor{\bsnm{Goldszmidt}, \binits{M.}}:
\bctitle{Properties and benefits of calibrated classifiers}.
In: \bbtitle{European Conference on Principles of Data Mining and Knowledge
  Discovery},
pp. \bfpage{125}--\blpage{136}
(\byear{2004}).
\bcomment{Springer}
\end{bchapter}
\endbibitem

%%% 51
\bibitem{song2021classifier}
\begin{botherref}
\oauthor{\bsnm{Song}, \binits{H.}},
\oauthor{\bsnm{Perello-Nieto}, \binits{M.}},
\oauthor{\bsnm{Santos-Rodriguez}, \binits{R.}},
\oauthor{\bsnm{Kull}, \binits{M.}},
\oauthor{\bsnm{Flach}, \binits{P.}}, et al.:
Classifier calibration: How to assess and improve predicted class
  probabilities: a survey.
arXiv preprint arXiv:2112.10327
(2021)
\end{botherref}
\endbibitem

%%% 52
\bibitem{kumar2019verified}
\begin{botherref}
\oauthor{\bsnm{Kumar}, \binits{A.}},
\oauthor{\bsnm{Liang}, \binits{P.S.}},
\oauthor{\bsnm{Ma}, \binits{T.}}:
Verified uncertainty calibration.
Advances in Neural Information Processing Systems
\textbf{32}
(2019)
\end{botherref}
\endbibitem

%%% 53
\bibitem{platt20005}
\begin{botherref}
\oauthor{\bsnm{Platt}, \binits{J.C.}}:
5 probabilities for sv machines.
Advances in Large Margin Classifiers,
61
(2000)
\end{botherref}
\endbibitem

%%% 54
\bibitem{leathart2017probability}
\begin{bchapter}
\bauthor{\bsnm{Leathart}, \binits{T.}},
\bauthor{\bsnm{Frank}, \binits{E.}},
\bauthor{\bsnm{Holmes}, \binits{G.}},
\bauthor{\bsnm{Pfahringer}, \binits{B.}}:
\bctitle{Probability calibration trees}.
In: \bbtitle{Asian Conference on Machine Learning},
pp. \bfpage{145}--\blpage{160}
(\byear{2017}).
\bcomment{PMLR}
\end{bchapter}
\endbibitem

%%% 55
\bibitem{guo2017calibration}
\begin{bchapter}
\bauthor{\bsnm{Guo}, \binits{C.}},
\bauthor{\bsnm{Pleiss}, \binits{G.}},
\bauthor{\bsnm{Sun}, \binits{Y.}},
\bauthor{\bsnm{Weinberger}, \binits{K.Q.}}:
\bctitle{On calibration of modern neural networks}.
In: \bbtitle{International Conference on Machine Learning},
pp. \bfpage{1321}--\blpage{1330}
(\byear{2017}).
\bcomment{PMLR}
\end{bchapter}
\endbibitem

%%% 56
\bibitem{ovadia2019can}
\begin{botherref}
\oauthor{\bsnm{Ovadia}, \binits{Y.}},
\oauthor{\bsnm{Fertig}, \binits{E.}},
\oauthor{\bsnm{Ren}, \binits{J.}},
\oauthor{\bsnm{Nado}, \binits{Z.}},
\oauthor{\bsnm{Sculley}, \binits{D.}},
\oauthor{\bsnm{Nowozin}, \binits{S.}},
\oauthor{\bsnm{Dillon}, \binits{J.}},
\oauthor{\bsnm{Lakshminarayanan}, \binits{B.}},
\oauthor{\bsnm{Snoek}, \binits{J.}}:
Can you trust your model's uncertainty? evaluating predictive uncertainty under
  dataset shift.
Advances in neural information processing systems
\textbf{32}
(2019)
\end{botherref}
\endbibitem

%%% 57
\bibitem{brocker2007increasing}
\begin{barticle}
\bauthor{\bsnm{Br{\"o}cker}, \binits{J.}},
\bauthor{\bsnm{Smith}, \binits{L.A.}}:
\batitle{Increasing the reliability of reliability diagrams}.
\bjtitle{Weather and forecasting}
\bvolume{22}(\bissue{3}),
\bfpage{651}--\blpage{661}
(\byear{2007})
\end{barticle}
\endbibitem

%%% 58
\bibitem{gupta2021distribution}
\begin{bchapter}
\bauthor{\bsnm{Gupta}, \binits{C.}},
\bauthor{\bsnm{Ramdas}, \binits{A.}}:
\bctitle{Distribution-free calibration guarantees for histogram binning without
  sample splitting}.
In: \bbtitle{International Conference on Machine Learning},
pp. \bfpage{3942}--\blpage{3952}
(\byear{2021}).
\bcomment{PMLR}
\end{bchapter}
\endbibitem

%%% 59
\bibitem{nixon2019measuring}
\begin{bchapter}
\bauthor{\bsnm{Nixon}, \binits{J.}},
\bauthor{\bsnm{Dusenberry}, \binits{M.W.}},
\bauthor{\bsnm{Zhang}, \binits{L.}},
\bauthor{\bsnm{Jerfel}, \binits{G.}},
\bauthor{\bsnm{Tran}, \binits{D.}}:
\bctitle{Measuring calibration in deep learning.}
In: \bbtitle{CVPR Workshops},
vol. \bseriesno{2}
(\byear{2019})
\end{bchapter}
\endbibitem

%%% 60
\bibitem{posocco2021estimating}
\begin{bchapter}
\bauthor{\bsnm{Posocco}, \binits{N.}},
\bauthor{\bsnm{Bonnefoy}, \binits{A.}}:
\bctitle{Estimating expected calibration errors}.
In: \bbtitle{International Conference on Artificial Neural Networks},
pp. \bfpage{139}--\blpage{150}
(\byear{2021}).
\bcomment{Springer}
\end{bchapter}
\endbibitem

%%% 61
\bibitem{villani2009optimal}
\begin{bbook}
\bauthor{\bsnm{Villani}, \binits{C.}}:
\bbtitle{Optimal Transport: Old and New}
vol. \bseriesno{338}.
\bpublisher{Springer}, \blocation{???}
(\byear{2009})
\end{bbook}
\endbibitem

%%% 62
\bibitem{peyre2019computational}
\begin{barticle}
\bauthor{\bsnm{Peyr{\'e}}, \binits{G.}},
\bauthor{\bsnm{Cuturi}, \binits{M.}}, \betal:
\batitle{Computational optimal transport: With applications to data science}.
\bjtitle{Foundations and Trends{\textregistered} in Machine Learning}
\bvolume{11}(\bissue{5-6}),
\bfpage{355}--\blpage{607}
(\byear{2019})
\end{barticle}
\endbibitem

%%% 63
\bibitem{he2016deep}
\begin{bchapter}
\bauthor{\bsnm{He}, \binits{K.}},
\bauthor{\bsnm{Zhang}, \binits{X.}},
\bauthor{\bsnm{Ren}, \binits{S.}},
\bauthor{\bsnm{Sun}, \binits{J.}}:
\bctitle{Deep residual learning for image recognition}.
In: \bbtitle{Proceedings of the IEEE Conference on Computer Vision and Pattern
  Recognition},
pp. \bfpage{770}--\blpage{778}
(\byear{2016})
\end{bchapter}
\endbibitem

%%% 64
\bibitem{hua2005optimal}
\begin{barticle}
\bauthor{\bsnm{Hua}, \binits{J.}},
\bauthor{\bsnm{Xiong}, \binits{Z.}},
\bauthor{\bsnm{Lowey}, \binits{J.}},
\bauthor{\bsnm{Suh}, \binits{E.}},
\bauthor{\bsnm{Dougherty}, \binits{E.R.}}:
\batitle{Optimal number of features as a function of sample size for various
  classification rules}.
\bjtitle{Bioinformatics}
\bvolume{21}(\bissue{8}),
\bfpage{1509}--\blpage{1515}
(\byear{2005})
\end{barticle}
\endbibitem

%%% 65
\bibitem{vergara2014review}
\begin{barticle}
\bauthor{\bsnm{Vergara}, \binits{J.R.}},
\bauthor{\bsnm{Est{\'e}vez}, \binits{P.A.}}:
\batitle{A review of feature selection methods based on mutual information}.
\bjtitle{Neural computing and applications}
\bvolume{24}(\bissue{1}),
\bfpage{175}--\blpage{186}
(\byear{2014})
\end{barticle}
\endbibitem

%%% 66
\bibitem{zeng2000distribution}
\begin{barticle}
\bauthor{\bsnm{Zeng}, \binits{X.}},
\bauthor{\bsnm{Martinez}, \binits{T.R.}}:
\batitle{Distribution-balanced stratified cross-validation for accuracy
  estimation}.
\bjtitle{Journal of Experimental \& Theoretical Artificial Intelligence}
\bvolume{12}(\bissue{1}),
\bfpage{1}--\blpage{12}
(\byear{2000})
\end{barticle}
\endbibitem

%%% 67
\bibitem{kuhn2013applied}
\begin{bbook}
\bauthor{\bsnm{Kuhn}, \binits{M.}},
\bauthor{\bsnm{Johnson}, \binits{K.}}, \betal:
\bbtitle{Applied Predictive Modeling}
vol. \bseriesno{26}.
\bpublisher{Springer}, \blocation{???}
(\byear{2013})
\end{bbook}
\endbibitem

%%% 68
\bibitem{kendall1938new}
\begin{barticle}
\bauthor{\bsnm{Kendall}, \binits{M.G.}}:
\batitle{A new measure of rank correlation}.
\bjtitle{Biometrika}
\bvolume{30}(\bissue{1/2}),
\bfpage{81}--\blpage{93}
(\byear{1938})
\end{barticle}
\endbibitem

%%% 69
\bibitem{platt1999probabilistic}
\begin{barticle}
\bauthor{\bsnm{Platt}, \binits{J.}}, \betal:
\batitle{Probabilistic outputs for support vector machines and comparisons to
  regularized likelihood methods}.
\bjtitle{Advances in large margin classifiers}
\bvolume{10}(\bissue{3}),
\bfpage{61}--\blpage{74}
(\byear{1999})
\end{barticle}
\endbibitem

\end{thebibliography}

